Reconfigurable Interaction for MAS Modelling

We propose a formalism to model and reason about multi-agent systems. We allow agents to interact and communicate in different modes so that they can pursue joint tasks; agents may dynamically synchronize, exchange data, adapt their behaviour, and reconfigure their communication interfaces. The formalism defines a local behaviour based on shared variables and a global one based on message passing. We extend LTL to be able to reason explicitly about the intentions of the different agents and their interaction protocols. We also study the complexity of satisfiability and model-checking of this extension.

==> tex/lowerbound.tex <==
% !TEX root = ../main.tex
\section{Lower Bound Complexity}\label{sec:lower}\marginpar{Y: In progress...}
In this section we investigate the hardness of \ltal satisfiability
and model-checking. In the previous section we showed that
satisfiability and model-checking problems are in EXPSPACE with
respect to common variables $\scv$. We now show that by a reduction
from EXPSPACE tiling problem~\cite{Wang90,Boas97} that satisfiability and
model-checking are EXPSPACE-hard. 

\begin{theorem}[hardness]
	\label{thm:hardness}
The satisfiability and model-checking problems for properties in \ltal are EXPSPACE-hard.
\end{theorem}

\begin{proof}
We provide a proof by showing a reduction form a version of the
EXPSPACE tiling problem~\cite{Wang90,Boas97}. In the EXPSPACE tiling problem, we
are given a set of tiles $T$, for convenience of encoding we assume
that $\size{T}=\Exp{n}$, a vertical and
horizontal relations $Y\subseteq T^2$ and $X\subseteq T^2$, an initial
tile $t_0$, a final tile $t_e$, and an integer $m>0$ encoded in
unary.
A solution to the tiling problem is $f:\{0,\ldots, \Exp{m}-1\} \times \{0,
\ldots, k\} \rightarrow T$ such that (a) $f(0,0)=t_0$, (b)
$f(\Exp{m}-1,k)=t_e$, (c) for every $k'\leq k$ and every $0<j<\Exp{m}$ we have
$(f(j-1,k'),(f(j,k'))\in X$, and (d) for every $0<k'\leq k$ and every
$0\leq k<\Exp{m}$ we have $(f(j,k'-1),f(j,k'))\in Y$.
The decision problem is to decide whether for some $k\geq 0$ there
exists such a solution.

We set up the satisfiability problem of an \ltal formula such that the
\ltal formula has an infinite computation satisfying it iff the tiling
problem has a solution. Thus, the satisfiability of \ltal is
EXPSPACE-hard.
Every state in the computation encodes one tile and its location
module $\Exp{m}$ (i.e., a number in $\{0,\ldots, \Exp{m}-1\}$). The
difficulty is in verifying the vertical consistency rules ((d)
above).

The formula relates to the propositions $\cn_1,\ldots, \cn_m$ encoding
the location of the tile in binary (current number), $\pn_1,\ldots, \pn_m$ encoding the
location of the previous tile in binary (previous number),
$\ct_1,\ldots, \ct_n$ encoding the tile in binary (current tile), and
$\pt_1,\ldots, \pt_n$ encoding the previous tile in binary (previous
tile).
We set up the possible truth assignments to these propositions so that
they indeed encode the locations of the tiles as well as use them to
check that the first tile is $t_0$, the ``last'' tile is $t_e$ and
that horizontal consistency rules hold.
We use the notation $\enccn{i}$ to refer to the Boolean formula that
says that the truth assignmnets to the propositions in $\cn$ encode
the value $i$. For example, $\bigwedge_{i=1}^m\neg \cn_i$ encodes the
number 0 and $\bigwedge_{i=1}^m \cn_i$ encodes the number $\Exp{m}-1$.
Similarly, we use the notations $\encpn{i}$, $\encct{t}$, and
$\encpt{t}$ to describe the encoding numbers using $\pn$ and the tile
$t$ using the propositions $\ct$ and $\pt$. 
Formally, we have the following parts of the final formula:
\begin{compactitem}
\item
  The propositions $\cn$ and $\pn$ encode the number of the current
  and previous locations:
  \begin{compactitem}
  \item
    The first tile is numbered $0$ and the previous number is $\Exp{m}-1$:
    \[\varphi_{1,1}=\enccn{0}\wedge\encpn{\Exp{m}-1}\]
  \item
    The next encoding of previous number copies the encoding of current number:
    \[\varphi_{1,2}=\g\band{\id=1}{m}{\cn_{\id}\Iff\nxt{\true}\pn_{\id}}\]
  \item
    After the number $\Exp{m}-1$ appears the number $0$. 
    \[\varphi_{1,3}=\g\tuple{\enccn{\Exp{m}-1}\Impl \nxt{\true}\enccn{0}}\]
%  \item
%    The least significant bit in $\cn$ toggles.
%    \[\varphi_{1,4}=\g\tuple{\cn_1\Iff\nxt{\true}\neg\cn_1}\]
  \item
    If currently all the bits lower than $i$ are true then the $i$-th
    bit toggles for the next number.  In particular, the least significant bit always toggles.
    \[\varphi_{1,4}=\g\tuple{\band{\id=1}{m}{\tuple{\band{\id'<\id}{}{\cn_{\id'}}\Impl\tuple{\cn_{\id}\Iff\nxt{\true}\neg\cn_{\id}}}}}\]
  \item
    If currently some bit lower than $i$ is false then the $i$-th bit
    does not change for the next number.
    \[\varphi_{1,5}=\g\tuple{\band{\id=2}{m}{\tuple{\bor{\id'<\id}{}{\neg\cn_{\id'}}\Impl\tuple{\cn_{\id}\Iff\nxt{\true}\cn_{\id}}}}}\]
  \end{compactitem}
  Let $\varphi_1=\bigwedge_{i=1}^5\varphi_{1,i}$. Then, every
  computaton satisfying $\varphi_1$ has the propositions in $\cn$ and
  $\pn$ encoding the current location modulo $\Exp{m}$ and the
  previous location modulo $\Exp{m}$.
\item
  Another part of the setup is that the encoding of the previous tile
  works as expected:
  \[\varphi_2=\g\band{\id=1}{n}{\ct_{\id}\Iff\nxt{\true}\pt_{\id}}\]
\item
  We now turn to encoding the start with $t_0$, end with $t_e$, and
  the horizontal consistency of the tiling.
  \begin{compactitem}
  \item
  The first tile encodes $t_0$:
  \[\varphi_{3,1}=\encct{t_0}\] 
  \item
    Let $\mathsf{End}\equiv\encct{t_e}\wedge\enccn{\Exp{m}-1}$. 
    Then, the following formula encodes both that $t_e$ appears
    somewhere in a location numbered by $\Exp{m}-1$ and that up to that
    location horizontal consistency rules hold:
  \[\varphi_{3,2}=\tuple{
    \neg\enccn{\Exp{m}-1}\Impl\bor{\tuple{t_1, t_2}\in
      X}{}{\encct{t_1}\wedge\nxt{\true}\encct{t_2}}}\ \Until
  \ \mathsf{End}\]
  \end{compactitem}
  Let $\varphi_3=\varphi_{3,1}\wedge\varphi_{3,2}$. Then, every
  computation satisfying $\varphi_3$ starts with the tile $t_0$ has
  the tile $t_e$ appearing in a location numbered $\Exp{m}-1$ and
  every two adjacent tiles (except the boundary between $\Exp{m}-1$
  and $0$) satisfy the horizontal consistency rules.
\item
  We now turn to encoding the vertical consistency rules. Here, for
  the first time, we will use the observation descriptors.
  First, we specify the data variables and the common variables.

  For the data variables, we copy the propositions. Thus, we have the
  sets of data variables $\{\dcn_1,\ldots, \dcn_m\}$,
  $\{\dpn_1,\ldots, \dpn_m\}$, $\{\dct_1,\ldots, \dct_n\}$, and
  $\{\dpt_1,\ldots, \dpt_n\}$ standing for \emph{data current number},
  \emph{data previous number}, \emph{data current tile}, and
  \emph{data previous tile}.

  For the communication varialbes, we enable to encode a number and a
  tile. Namely, $\{cvn_1,\ldots,\cvn_m\}$ and $\{\cvt_1,\ldots,
  \cvt_n\}$ are common variables that enable to encode a number and a
  tile, respectively. Recall that a predicate over $\cv$ encodes a set
  of possible assignments to $\cv$. Thus, we can think about such a
  predicate as a relation $R\subseteq \{0,\ldots, \Exp{m}-1\}\times
  T$.
  We will add formulas that ensure that the predicate actually encodes
  a function $R:\{0,\ldots,\Exp{m}-1\}\rightarrow T$ and effectively,
  the predicate characterizes exactly the contents of the previous
  $\Exp{m}$ tiles allowing us to check the vertical consistency rules.
  We use the notation $R_\pi$ for referring to the relation encoded by
  the predicate in the observation and $R'_\pi$ for the relation
  encoded by the predicate in the next observation.
  We write $(i,t)\in R_\pi$ to mean
  the assignment that associates the number $i$ with the tile $i$ is
  allowed by $R_\pi$. We also use $\cn$ to refer to the number encoded
  by the propositions $\cn$ and similarly for other
  propositions/variables. 
  \begin{compactitem}
    \item
      The data variables copy the values of the propositions:
      \[
      \varphi_{4,1}=\g\tuple{\begin{array}{l c l l}
          \band{\id=1}{n}{\tuple{\ct_{\id}\Iff\nxt{\dct_{\id}}\true}}
          \wedge \

\band{\id=1}{n}{\tuple{\pt_{\id}\Iff\nxt{\dpt_{\id}}\true}}
\wedge \

\band{\id=1}{m}{\tuple{\cn_{\id}\Iff\nxt{\dcn_{\id}}\true}}
\wedge \\[2ex]

\band{\id=1}{m}{\tuple{\pn_{\id}\Iff\nxt{\dpn_{\id}}\true}}
\end{array}}
\]
\item
  We now set up the $R_\pi$ to encode a function that correctly memorizes
  the tiles in the previous $\Exp{m}$ locations. Thus, if $R_\pi$
  appears in the observation
  happening after a location numered $i$ then $R_\pi$ encodes the
  tiles in locations $i$ to $\Exp{m}-1$ in the previous ``line'' and the
  locations $0$ to $i-1$ in the same ``line''.
  \begin{compactitem}
  \item
    Relation $R_\pi$ includes the assignment that encodes the previous
    tile associated with the previous number. That is $(\pn,\pt)\in R_\pi$
    \[
    \varphi_{4,2,1}=\nxt{\true}\g\tuple{\bnxt{\exis{\tuple{\begin{array}{l c l l}
              \band{\id=1}{m}{\cvn_{\id}\Iff\dpn_{\id}}\wedge\\
              \band{\id=1}{n}{\cvt_{\id}\Iff\dpt_{\id}}
            \end{array}
      }}}\true}
    \]
  \item
    The predicate allows only for the assignment that encodes the
    previous tile associated with the previous number.
    That is, if for some $t$ we have $(\pn,t)\in R_\pi$ then $t=\pt$. 
  \[\varphi_{4,2,2}=
  \nxt{\true}\g\tuple{\bnxt{\all{\tuple{\begin{array}{l c l l}
            \band{\id=1}{m}{\cvn_{\id}\Iff\dpn_{\id}}\Impl\\
            \band{\id=1}{n}{\cvt_{\id}\Iff\dpt_{\id}}
          \end{array}
    }}}\true}
  \]
\item
  For every tile $t$, if for some $v\neq \cn$ such that the $j$-th bit of $v$ is
  true we have $(v,t)\in R_{\pi}$ then there is some $v'\neq \cn$ such
  that the $j$-th bit of $v'$ is true as well and $(v',t)\in
  R'_{\pi}$.
\[
\varphi_{4,2,3,j}=\g{\tuple{
\begin{array}{l c l l}
\band{t\in T}{}{\anglebr{\exis{\tuple{\begin{array}{l c l l}
\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dcn_{\id}\xor\cvn_{\id}}
\end{array}
}}}
\bnxt{\exis{\tuple{\begin{array}{l c l l}
\cvn_j\wedge\\
\enccvt{t}\ \wedge\\
\bor{\id=1}{m}{\dpn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\true\ \wedge}\\[8ex]

\begin{array}{l c l l}
\band{t\in T}{}{\alws{\true}\anglebr{\exis{\tuple{\begin{array}{l c l l}
\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dpn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\false\ \lor\ 
\bnxt{\exis{\tuple{\begin{array}{l c l l}
\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dcn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\true}
\end{array}
\end{array}
}}
\]
\item
  For every tile $t$, if for some $v\neq \cn$ such that the $j$-th bit of $v$ is
  false we have $(v,t)\in R_{\pi}$ then there is some $v'\neq \cn$ such
  that the $j$-th bit of $v'$ is false as well and $(v',t)\in
  R'_{\pi}$.
\[
\varphi_{4,2,4,j}=\g{\tuple{
\begin{array}{l c l l}
\band{t\in T}{}{\anglebr{\exis{\tuple{\begin{array}{l c l l}
\neg\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dcn_{\id}\xor\cvn_{\id}}
\end{array}
}}}
\bnxt{\exis{\tuple{\begin{array}{l c l l}
\neg\cvn_j\wedge\\
\enccvt{t}\ \wedge\\
\bor{\id=1}{m}{\dpn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\true\ \wedge}\\[8ex]

\begin{array}{l c l l}
\band{t\in T}{}{\alws{\true}\anglebr{\exis{\tuple{\begin{array}{l c l l}
\neg\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dpn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\false\ \lor\ 
\bnxt{\exis{\tuple{\begin{array}{l c l l}
\neg\cvn_j\wedge\\
\enccvt{t}\wedge\\
\bor{\id=1}{m}{\dcn_{\id}\xor\cvn_{\id}}
\end{array}
}}}\true}
\end{array}
\end{array}
}}
\]
\end{compactitem}
Consider now the conjunction $\varphi_{4,2}=\varphi_{4,2,1}\wedge
\varphi_{4,2,2}\wedge \bigwedge_{j=1}^m (\varphi_{4,2,3,j}\wedge
\varphi_{4,2,4,j})$.
By $\varphi_{4,2,1}$ and $\varphi_{4,2,2}$ we know that in a location
$i$ we have that $R_\pi$ correctly encodes the previous tile with the
previous number and only that tile is associated with that number.
Now consider the set of tiles $T_{i'}$ that are associated with a number
$i'\neq i$ in $R_\pi$. The rest of the conjunction establishes that
the same set of tiles is associated with $i'$ in $R'_\pi$.

Conisder a bit $j$, let $R_\pi(j,\true)$ denote the set of tiles that are
associated with numbers whose $j$-th bit is true and similarly
$R_\pi(j,\true)$.
Let $R_\pi(i')$ denote the set of tiles associated with $i'$ in
$R_\pi$.
Let $i'_j$ denote the $j$-th bit of $i'$.

Then, $R_\pi(i') \subseteq \bigcap_{j=1}^m R_\pi(j,i'_j)$.
Consider a tile appearing in $blah$
\item
  Finally, we can encode the vertical consistency. Let
\[
\mathsf{Vertical}\equiv\bor{\tuple{t_1, t_2}\in Y}{}{\bnxt{\exis{\tuple{\begin{array}{l c l l}
\band{\id=1}{m}{\cvn_{\id}\Iff\dcn_{\id}}\wedge\\
\encdct{t_2}\wedge\enccvt{t_1}
\end{array}
}}}\true}
\]
$\mathsf{Vertical}$ essentially says that the current tile is
vertically associated with the unique tile in $R_\pi$ that has the
current number. That is, the tile that appears exactly $\Exp{m}$
locations before the current tile.

Finally, we have to ensure that vertical consistency holds from the
second appearance of the number $0$ until the appearance of $t_e$ and
that $t_e$ itself is also vertically consistent. 
\[
\varphi_{4,3}=\nxt{\true}\tuple{\neg\enccn{0}\ \Until\ \tuple{\enccn{0}\wedge\tuple{\mathsf{Vertical}\ \Until\ \tuple{\mathsf{End}\wedge\mathsf{Vertical}}}}}
\]
  \end{compactitem}
  It follows that $\varphi_4=\bigwedge_{j=1}^3\varphi_{4,j}$ completes
  the encoding.
\end{compactitem}

Let $\varphi=\bigwedge_{j=1}^4\varphi_i$.

\begin{lemma}
  The formula $\varphi$ is satisfiable if and only if the tiling
  problem $T$ has a solution. 
\end{lemma}

\begin{proof}
  This follows from the explanations above. 
\end{proof}
\end{proof}


==> tex/relatedwork.tex <==
% !TEX root = ../main.tex
\section{Related work}\label{sec:rel}

%\marginpar{Y: compare with respect to other models arising in verification and concurrency theory communities}
%
\paragraph*{System frameworks}
The modelling of computer systems in terms of interacting and distributed components is a well established approach in the area of formal verification that has recently been imported to multi-agent settings~\cite{Woo02,WGHMPT16,GHW17,KL17a,KL17b}.
One of the most successful formalisms in this area is the one of Reactive Modules~\cite{AH99b}, a high-level language for the specification of components capabilities in terms of guarded commands: variable assignment rules that activate/deactivate according to a guarded predicate evaluated on the current state of the system.

Antithetical to the traditional communication framework, the interaction among components is based exclusively on shared variables, whereas the message-exchange is assumed both implicit and instantaneous.
More recently, an extension to \emph{Dynamic Reactive Modules}~\cite{FHNPSV11} accounts for communication reconfigurability, where processes can evolve their set of guarded commands, as well as being created or terminated.
Other extensions of reactive modules account for scenarios in which variables are not visible to all the components~\cite{GPW18}, or such visibility is dynamically disclosed or concealed by the controller itself~\cite{BBDM19}, again allowing the communication mechanism to reconfigure.

%\marginpar{Y: compare with other existing logics and justify the need for another logic}
%
\paragraph*{Logics}
In reactive modules verification, the specification language for system correctness is usually logic-based.
In particular, LTL and CTL like languages are well established formalisms for the representation of temporal properties in systems executions.
However, such languages are not suitable to specify properties for the modalities on which transitions among systems states are triggered.
Therefore, in order to predicate over the message-passing architecture, one has to consider extensions or variations that are capable to constrain the transition relation of systems.
Existing languages of this kind include \emph{Propositional Dynamic Logic}~\cite{FL79} and \emph{modal $\mu$-calculus}~\cite{Koz83}.

Unfortunately, these languages are still limited for our purpose, as they treat the transition labels as atomic objects, whereas our system models mount complex and structured observations on which designers are willing to predicate on.
In order to verify such articulated properties along them, we need a modal language whose modalities adapt over the space of possible observations.
As we show in here, such extension comes with an unavoidable price in the complexity of the model-checking problem.




==> tex/varstyles.tex <==
%% !TEX root = ../main.tex
\newcommand{\sqt}[1]{`{#1}'}
\newcommand{\keep}{\mbox{\sc keep}}
% agents
\newcommand{\agent}[1]{\rulename{\textbf{#1}}}
\newcommand{\lineagent}{\agent{Line}}
\newcommand{\taagent}{\agent{t1}}
\newcommand{\tbagent}{\agent{t2}}
\newcommand{\tcagent}{\agent{t3}}

% variable types macros
\newcommand{\varcommon}[1]{\footnotesize{\text{@}}\mathsf{#1}}
\newcommand{\vardata}[1]{\rulename{#1}} 
\newcommand{\varlocal}[1]{\mathsf{#1}}
\newcommand{\val}[1]{{\small{\texttt{#1}}}}

% common variables
\newcommand{\typecvar}{\varcommon{type}}
\newcommand{\assigncvar}{\varcommon{asgn}}
\newcommand{\readycvar}{\varcommon{rdy}}

% data variables
\newcommand{\msgdvar}{\vardata{msg}}
\newcommand{\lnkdvar}{\vardata{lnk}}
\newcommand{\nodvar}{\vardata{no}}

% line variables
\newcommand{\stlvar}{\varlocal{st}}
\newcommand{\lnklvar}{\varlocal{lnk}}
\newcommand{\prdlvar}{\varlocal{prd}}
\newcommand{\stagelvar}{\varlocal{stage}}
\newcommand{\typelvar}{\varlocal{ltype}}
\newcommand{\assignlvar}{\varlocal{lasgn}}
\newcommand{\readylvar}{\varlocal{lrdy}}

% variable values
\newcommand{\taval}{\val{t1}}
\newcommand{\tbval}{\val{t2}}
\newcommand{\tcval}{\val{t3}}
\newcommand{\teamval}{\val{team}}
\newcommand{\assembleval}{\val{asmbl}}
\newcommand{\formval}{\val{form}}
\newcommand{\pendval}{\val{pnd}}
\newcommand{\recval}{\val{rcrt}}
\newcommand{\stageoneval}{\val{stg1}}
\newcommand{\stagetwoval}{\val{stg2}}
\newcommand{\startval}{\val{strt}}
\newcommand{\recother}{\val{rec\_oth}}
